Deep-learning-based surrogate flow modeling and geological parameterization for data assimilation in 3D subsurface flow

Data assimilation in subsurface flow systems is challenging due to the large number of flow simulations often required, and by the need to preserve geological realism in the calibrated (posterior) models. In this work we present a deep-learning-based surrogate model for two-phase flow in 3D subsurface formations. This surrogate model, a 3D recurrent residual U-Net (referred to as recurrent R-U-Net), consists of 3D convolutional and recurrent (convLSTM) neural networks, designed to capture the spatial-temporal information associated with dynamic subsurface flow systems. A CNN-PCA procedure (convolutional neural network post-processing of principal component analysis) for parameterizing complex 3D geomodels is also described. This approach represents a simplified version of a recently developed supervised-learning-based CNN-PCA framework. The recurrent R-U-Net is trained on the simulated dynamic 3D saturation and pressure fields for a set of random `channelized' geomodels (generated using 3D CNN-PCA). Detailed flow predictions demonstrate that the recurrent R-U-Net surrogate model provides accurate results for dynamic states and well responses for new geological realizations, along with accurate flow statistics for an ensemble of new geomodels. The 3D recurrent R-U-Net and CNN-PCA procedures are then used in combination for a challenging data assimilation problem involving a channelized system. Two different algorithms, namely rejection sampling and an ensemble-based method, are successfully applied. The overall methodology described in this paper may enable the assessment and refinement of data assimilation procedures for a range of realistic and challenging subsurface flow problems.

==> chap0.tex <==

\textcolor{blue}{In recent work, we have developed deep-learning-based procedures for parameterizing complex 2D geomodels and for predicting the detailed flow responses of such systems. The parameterization method, referred to as CNN-PCA, entails the use of principal component analysis in combination with convolutional neural networks, while the flow surrogate model involves the application of a recurrent residual U-Net procedure. The combination of these two capabilities enables efficient history matching to be performed. This is because the variables that must be determined during data assimilation correspond to the relatively small set of parameters associated with the CNN-PCA description, and the requisite flow simulations can all be accomplished using the deep-learning-based surrogate model. The overall methodology has been successfully applied to 2D channelized systems. In this work, we extend these capabilities to 3D systems. The 3D CNN-PCA procedure differs from the 2D method in that we no longer use a style loss term (as we did in 2D), but instead apply a supervised learning approach. With this method we train the network using PCA realizations along with their corresponding (desired) channelized representations. This treatment, in common with our 2D procedure, leads to faster training than some other approaches since the underlying PCA representation already captures aspects of the spatial statistics (covariance). The 3D recurrent R-U-Net consists of 3D convolutional and recurrent (convLSTM) neural networks, which are designed to capture the spatial and temporal information associated with dynamic systems. This approach shows advantages over autoregressive procedures. The recurrent R-U-Net is trained on 2500 randomly generated 3D geomodels and their corresponding (simulated) dynamic 3D state maps; e.g., saturation and pressure at a set of time steps. Results are first presented for each method individually. Specifically, we validate the geological parameterization procedure by demonstrating that the prior flow statistics, for a 3D channelized system, generated using CNN-PCA agree closely with those from (reference) geostatistical models. The recurrent R-U-Net surrogate flow model is validated through detailed comparisons of oil-water flow results for particular (new) realizations and through error statistics for an ensemble of new models. Finally, a 3D history matching example, in which 3D CNN-PCA and recurrent R-U-Net are applied with rejection sampling and an ensemble-based method, are presented. High-fidelity simulation results for the accepted posterior models of rejection sampling are in close agreement with the surrogate predictions. And substantial uncertainty reduction is observed after the rejection sampling procedure. The posterior uncertainty of the ensemble-based method is overestimated for some well response quantities when compared with the rigorous rejection sampling methods. And the use of 3D CNN-PCA and recurrent R-U-Net in combination enables effective evaluations of different history matching algorithms. }



==> chap1.tex <==
\section{Introduction}

History matching entails the calibration of geological model parameters such that flow simulation predictions are in essential agreement with historical (observed) data. The prediction uncertainty associated with these calibrated (posterior) models is typically less than that from the initial (prior) models, which renders them more useful for reservoir management. History matching involves many challenges, including the preservation of geological realism in posterior models, and the computational demands associated with the requisite flow simulations. Thus this application will benefit from the development and use of effective geological parameterizations and accurate surrogate models for flow predictions. 


\textcolor{blue}{The advance of deep learning in the past decades has revolutionized fields of image recognition~\citep{simonyan2014very, he2016deep} and natural language processing~\citep{collobert2008unified, devlin2018bert}, and nowdays its influence has expanded to physics and engineering field, and many successful applications~\citep{tian2020surrogate, zhang2020self, weinan2018deep, lu2019deepxde, iten2020discovering,raissi2020hidden, berg2018unified} demonstrated the potentials of deep learning in supplementing and even replacing traditional engineering methods.} In recent work, a deep-learning-based geological parameterization technique, referred to as CNN-PCA~\citep{liu2019multilevel, liu2019deep}, and a surrogate flow model that applies a recurrent residual U-Net (R-U-Net) procedure, have been successfully applied for history matching 2D channelized systems~\citep{tang2020deep}. In this work, we extend these capabilities to 3D systems. The CNN-PCA parameterization enables the 3D geomodels to be described using relatively few variables, while the recurrent R-U-Net accurately captures the evolution of pressure and saturation fields, along with the well rates, for new models proposed during the history matching process. 

\textcolor{blue}{
Tools based on deep-learning have been shown to be applicable for the parameterization of complex geological patterns. Two most popular deep-learning techniques that have been successfully applied in geological parameterization include variational autoencoders~(VAEs)~\citep{Laloy2017, Canchumuni2019a} and generative adversarial networks~(GANs)~\citep{Chan2017, Chan2018, Dupont2018, Mosser2018, Laloy2018, Laloy2019, Chan2020, Azevedo2020}. There are also algorithms based on a combination of VAE and GAN, as demonstrated in \cite{mo2020integration}. Geological parameterization algorithms based on VAE and GAN establish an end-to-end mapping of geological models into low-dimensional latent variables. An alternative approach is to use deep-learning as a post-processor for traditional parameterization method, such as CNN-PCA \citep{liu2019deep} which use CNN to post-process low-dimensional PCA representations of geological models. In CNN-PCA, dimension reduction is off-loaded to PCA which reduces the computational burden of the training process of CNN. As a result, CNN-PCA in general requires less training samples and less training iterations comparing to algorithms based on VAE and GAN. However, the original 2D CNN-PCA formulation involves a transfer learning process where the VGG-net pretained for image classification is used for feature extraction of 2D geological models. In this study, we introduce an alternative surpervised-learning based loss function for CNN-PCA that extends naturally to 3D geological models and test our algorithm for parameterizing conditional geological models representing a 3D channelized system.
}

There have also been several deep-neural-network architectures proposed for surrogate flow modeling in subsurface systems. Zhu and Zabaras~\citep{zhu2018bayesian} devised a fully convolutional encoder-decoder architecture to capture pressure and velocity maps for single-phase flow problems characterized by random 2D Gaussian permeability fields. In subsequent work, an autoregressive strategy was integrated with a fully convolutional encoder-decoder architecture for the prediction of time-dependent contaminant transport in 2D problems \citep{mo2018deep}. Tang et al.~\citep{tang2020deep} later proposed a combination of a residual U-Net with convLSTM to capture the saturation and pressure evolution in 2D oil-water problems, with wells operating under wellbore pressure control. \textcolor{blue}{Mo et al.~\cite{mo2020integration} applied a 2D deep residual dense convolutional neural network to predict 3D groundwater solution concentration distributions, where the 3D output is a stack of 2D output channels. This treatment, however, ignores the geo-property correlation in the vertical direction and may not work well for complex 3D problems with many vertical layers. } Within the context of optimization (rather than history matching), Jin et al.~\citep{jin2020deep} presented an autoregressive embed-to-control framework to predict well responses and dynamic state evolution with varying well controls, for a fixed geological description.

\textcolor{blue}{The above deep learning-based surrogate modeling techniques all require input-output simulation data generated by traditional numerical methods to train the neural network. There are, however, physics informed surrogate modeling investigated where no simulation data is needed~\citep{raissi2019physics, han2018solving, sun2020surrogate, mao2020physics}. Governing partial differential equations~(PDEs) can be approximately solved by formulating the PDE residuals, as well as initial and boundary conditions as the minimizing objective for neural nets, as discussed in \citep{raissi2019physics}. However, there are many challenges needed to be addressed before this type of method can be used for complex coupled PDE problems, e.g., reservoir simulation in this study. The training difficulties increase significantly as the number of wells increases, which serves as boundary conditions in reservoir simulation. Heterogeneous discretized permeability maps, discontinuous initial and boundary conditions, which are common in traditional reservoir simulation, all need reformulating as smooth, continuous functions of time and space, before this method can be applied. More importantly, neural nets need to be retrained for every PDEs with the same form but different coefficient functions, which makes it inapplicable for surrogate modeling in history matching where many those PDEs need to be solved.} 

\textcolor{blue}{Zhu et al.~\cite{zhu2019physics} proposed a physics-constrained surrogate modeling for uncertainty quantification on high-dimension discretized fields, where a convolutional encoder-decoder surrogate can be trained to handle different discretized PDE coefficients, i.e., discretized permeability fields in reservoir simulation. This work incorporated an approximate governing PDE residual as training objective for a steady state problem. However, formulating the exact governing PDE residuals over discretized grids can be very challenging for complex reservoir problems, which has always been a demanding task in the development of traditional reservoir simulators~\citep{zhou2012parallel}. Meanwhile, the extension of this work to handle dynamic systems may be limited to explicit Euler method~(autoregressive strategy)~\citep{geneva2020modeling} in this framework. Although no simulation data is needed, these physics informed deep learning methods are not applicable for complex reservoir problems for various reasons~(mentiond above) in the current stage.  }

Extensions of these (and other) parameterization and surrogate flow modeling procedures to complex 3D systems are required before these techniques can be applied in practical settings. In this work we extend our earlier treatments to handle prototype 3D problems. Our 3D CNN-PCA differs from the 2D procedure, as we now use a supervised learning approach to map PCA models to `channelized' realizations. The 3D recurrent R-U-Net involves a similar layout to that used for 2D problems, but we now apply 3D CNN and convLSTM architectures. The 3D recurrent R-U-Net surrogate flow model is trained using flow results for realizations generated by 3D CNN-PCA.

%The 3D CNN-PCA is trained using O(3000) PCA realizations with their corresponding channelized representations generated by Petrel~\citep{manual2007petrel}. Different with 2D CNN-PCA in training loss setup, 3D CNN-PCA procedure introduces an alternative supervised learning approach which takes advantage of PCA's ability to approximate original models. The trained 3D CNN-PCA model can then be used to effectively generate diverse 3D high-dimensional channelized geological patterns by sampling low-dimensional PCA variables. The 3D recurrent R-U-Net is trained on O(2500) random 3D geomodels (generated by 3D CNN-PCA) and corresponding dynamic 3D maps. Well responses are further obtained by referring pressure and saturation at well blocks. 

This paper proceeds as follows. We first introduce the 3D CNN-PCA procedure and present geomodels generated using this technique. Flow results for an ensemble of random 3D CNN-PCA models are then compared to reference results from Petrel \citep{manual2007petrel} realizations. Next, we describe the deep-neural-network architecture and training setup for the 3D recurrent R-U-Net surrogate model. The method is validated by comparing oil-water flow predictions from the surrogate model to those from high-fidelity simulations. We then apply the 3D CNN-PCA and 3D recurrent R-U-Net models for a history matching problem. A rigorous rejection sampling method is used, with new realizations generated by 3D CNN-PCA and flow predictions provided by the 3D recurrent R-U-Net. We conclude with a summary and suggestions for future work.


% section
\section{3D CNN-PCA Formulation and Flow Results}

In this section we describe the 3D CNN-PCA procedure and present geomodels generated using this approach. We then compare flow responses from simulations using 3D CNN-PCA geomodels to those from reference Petrel realizations. 


%% subsection
\subsection{CNN-PCA Formulation}
A geological realization can be represented as a vector $\mathbf{m} \in \mathbb{R}^{n_b}$ of (isotropic) permeability values, where $n_b$ is the number of grid blocks in the model. Geological parameterizations map $\mathbf{m}$ to a new low-dimensional variable $\mathbf{\xi} \in \mathbb{R}^{l}$, where $l \ll n_b$. The first step in our procedure is to construct a PCA parameterization of the geomodel. As described in detail in \citep{liu2019deep}, this entails generating a set of $n_r$ realizations of $\mathbf{m}$, using geomodeling tools such as Petrel \citep{manual2007petrel}, and assembling these realizations in a centered data matrix $Y \in \mathbb{R}^{n_b \times n_r}$,
%
\begin{equation}
    \label{eq_center_data_matrix}
    Y = \frac{1}{\sqrt{n_r - 1}}[\mathbf{m}_1 - \bar{\mathbf{m}} \quad \mathbf{m}_2 - \bar{\mathbf{m}} \quad \cdots \quad \mathbf{m}_{n_r} - \bar{\mathbf{m}}],
\end{equation}
%
where $\mathbf{m}_i \in \mathbb{R}^{n_b}$ represents realization $i$ and $\bar{\mathbf{m}} \in \mathbb{R}^{n_b}$ is the mean of the $n_r$ prior realizations. Note that these realizations are all conditioned to available hard data at well locations. Singular value decomposition of $Y$ allows us to write $Y = U\Sigma V^{\intercal}$, where $U \in \mathbb{R}^{n_b \times n_r}$ and $V \in \mathbb{R}^{n_r \times n_r}$ are left and right singular matrices, and $\Sigma \in \mathbb{R}^{n_r \times n_r}$ is a diagonal matrix containing the singular values.

%Singular value decomposition of $Y$ allows us to write $Y = U\Sigma V^{\intercal}$, where $U \in \mathbb{R}^{n_b \times (n_r-1)}$ and $V \in \mathbb{R}^{n_r \times (n_r-1)}$ are left and right singular matrices, and $\Sigma \in \mathbb{R}^{(n_r-1) \times (n_r-1)}$ is a diagonal matrix containing the singular values.

New (PCA) realizations $\mathbf{m}_\text{pca} \in \mathbb{R}^{n_b}$ can be generated through application of
%
\begin{equation}
    \label{eq_pca}
    \mathbf{m}_\text{pca} = \Bar{\mathbf{m}} + U_l \Sigma_l \mathbf{\xi}_l,
\end{equation}
%
where $U_l \in \mathbb{R}^{n_b \times l}$ contains the $l$ columns in $U$ associated with the largest singular values 
%($l$ is the reduced dimension) 
and $\Sigma_l \in \mathbb{R}^{l \times l}$ contains the $l$ largest singular values. Standalone PCA provides accurate geomodels $\mathbf{m}_\text{pca}$ when the initial realizations $\mathbf{m}_i$ follow a multi-Gaussian distribution. With more complex spatial statistics, PCA does not fully preserve the features appearing in $\mathbf{m}_i$.

In CNN-PCA, we post-process PCA models using a deep convolutional neural network (CNN) to better preserve the complex spatial correlations. This post-processing, referred to as a model transform net, is represented as
%
\begin{equation}
    \label{eq_cnnpca_fw}
    \mathbf{m}_\text{cnnpca} = f_W(\mathbf{m}_\text{pca}),
\end{equation}
%
where $f_W$ indicates the model transform net and the subscript $W$ denotes the trainable weights. The training losses used in our 2D CNN-PCA \citep{liu2019deep} include a style loss term that is based on statistical quantities extracted from the VGG net \citep{simonyan2014very}. Since the VGG net only accepts image-like 2D inputs, it cannot be directly used for extracting features from 3D geological models. In this study, we therefore use an alternative supervised learning approach in 3D CNN-PCA.

% Our extension of CNN-PCA to 3D involves two main directions. One direction is replacing VGG-net with 3D CNN models such as the C3D net for video classification. Another direction is introducing a new loss term based on supervised learning. The combination of both approaches is shown to be the most effective. However, i

% The larger the reduced dimension $l$, the closer the reconstructed model $\hat{\mathbf{m}}_\text{pca}$ matches the original model $\mathbf{m}$. 

%xxx -- stopped editing here -- equations and descriptions need cleanup -- hats, tildes, subscripts 1 and 2, i consistently subscripted, describe hard data loss, ...

Our method proceeds as follows. Given an original geomodel $\mathbf{m}$, we map $\mathbf{m}$ onto the first $\hat{l}$ principal components,
%
\begin{equation}
\hat{\mathbf{\xi}}_{\hat{l}} = \Sigma^{-1}_{\hat{l}}U^T_{\hat{l}}(\mathbf{m} - \Bar{\mathbf{m}}).
\end{equation}
%
The model $\mathbf{m}$ can then be approximately reconstructed using
%
\begin{equation}
    \hat{\mathbf{m}}_\text{pca} = \Bar{\mathbf{m}} + U_{\hat{l}} \Sigma_{\hat{l}} \hat{\mathbf{\xi}}_{\hat{l}},
\end{equation}
%
where $\hat{\mathbf{m}}_\text{pca}\in \mathbb{R}^{n_b}$ is the reconstructed PCA model, and $\hat{l}$ is a low-dimensional variable such that $\hat{l} < l$ (for reasons explained below). The difference between $\hat{\mathbf{m}}_\text{pca}$ and the corresponding $\mathbf{m}$ can be viewed as the reconstruction error. The goal of the supervised training is to determine the parameters in the transform net $f_W$ such that this error is minimized. In other words, we seek to minimize the difference between $f_W(\hat{\mathbf{m}}_\text{pca})$ and $\mathbf{m}$. 

We use the same $n_r$ realizations of $\mathbf{m}$ as were used for constructing the PCA representation to generate the corresponding $\hat{\mathbf{m}}_\text{pca}^i$ models. This forms the training set, with each pair of $(\mathbf{m}^i, \hat{\mathbf{m}}_\text{pca}^i)$ representing one training sample. The supervised learning training loss for training sample $i$ is defined as
%
\begin{equation}
    L_\text{rec}^i = ||f_W(\hat{\mathbf{m}}_\text{pca}^i) - \mathbf{m}^i||_1.
\end{equation}
%
This quantity is referred to as the reconstruction loss.

Recall that, when 3D CNN-PCA is used to generate geomodels during history matching, this entails post-processing new PCA models $\mathbf{m}_\text{pca}(\mathbf{\xi}_l)$, with $\mathbf{\xi}_l$ sampled from the standard normal distribution. By using $\hat{l}<l$ during training, we make the reconstruction error more representative of what will be encountered at this (test) stage, where we do not have corresponding pairs $(\mathbf{m}^i, \hat{\mathbf{m}}_\text{pca}^i)$. We found this approach to lead to better performance at test time, when $f_W$ is applied for new PCA models.

We also include a hard data loss $L_\text{h}^i = [\mathbf{h}^T(\mathbf{m}^i-f_W(\hat{\mathbf{m}}_\text{pca}^i)]^2$ to (essentially) ensure that hard data are honored. Here $\mathbf{h}$ is an indicator vector, with $h_i=1$ indicating the presence of hard data at grid block $i$, and $h_i=0$ the absence of hard data. Note that hard data are captured in the PCA models, but without the inclusion of $L_\text{h}^i$ these data would not necessarily be maintained in the $\mathbf{m}_\text{cnnpca}$ models. The final training loss for training sample $i$ is now
%
\begin{equation}
    L^i = L_\text{rec}^i + \gamma_h L_\text{h}^i,
\end{equation}
%
where $\gamma_h$ is a weighting factor for the hard data loss. We determine $\gamma_h$ by considering a range of values and selecting a value that is sufficiently large such that essentially all hard data are honored in the output models. Specifically, in the example below, $\gamma_h$ is set such that, over all new 3D CNN-PCA geomodels, hard data in well blocks are honored more than 99.9\% of the time.

Construction of the 3D model transform net entails replacing the 2D convolutional layers, upsampling layers and padding layers in the 2D model transform net \citep{liu2019deep} with their 3D counterparts. This can be readily accomplished using the Pytorch deep-learning framework \citep{Paszke2017}. \textcolor{blue}{The architecture details of the 3D CNN-PCA transformer net is provided in Appendix~A.1.} In the case considered here, we generate $n_r=3000$ realizations of $\mathbf{m}$ using object-based modeling within Petrel. These models are then used to construct the PCA representation and to generate the corresponding $\hat{\mathbf{m}}_\text{pca}$ models. Based on limited numerical experimentation, we use a reduced dimension of $l=200$ for the new PCA models and a dimension of $\hat{l}=50$ for the reconstructed PCA models. The weighting factor for hard data loss is $\gamma_h = 0.02$. We use a batch size of 4 and train the model transform net for 10~epochs. This requires about 30~minutes using one Tesla V100 GPU. 

% with a training set of original models and reconstructed PCA models. The general architecture of $f_W$ for 3D CNN-PCA is identical to that used in \citep{liu2019deep}, which is composed of three conv blocks, five residual blocks and three transposed conv blocks, but with all 2D convolutional operations replaced with 3D convolutional operations. After training, we can generate new models efficiently by sampling $\mathbf{\xi}_l$ from $N(0,I_l)$, construct PCA model and post-process with $f_W$. %These new models can be combined with surrogate simulation model and rejection sampling for history matching and rigorous uncertainty estimation. 

% %
% \begin{equation}
% \hat{\mathbf{\xi}}_{l_2} = \Sigma^{-1}_{l_2}U^T_{l_2}(\mathbf{m} - \Bar{\mathbf{m}}),
% \end{equation}
% then we can reconstruct $\mathbf{m}$ with 
% \begin{equation}
%     \hat{\mathbf{m}}_\text{pca} = \Bar{\mathbf{m}} + U_{l_2} \Sigma_{l_2} \hat{\mathbf{\xi}}_{l_2}.
% \end{equation}
% With the same reduced dimension, the reconstructed PCA model $\hat{\mathbf{m}}_\text{pca} \in \mathbb{R}^{n_b}$ better preserves the spatial correlation than new PCA models $\mathbf{m}_\text{pca}$ (with $\mathbf{\xi}_l$ sampled from the standard Gaussian distribution). 
% % If we use the same dimension $l$, train $f_W$ on $\hat{\mathbf{m}}_\text{pca}$ and later evaluate on $\mathbf{m}_\text{pca}$ during history matching, the resulted model will not preserve the spatial correlation of $\mathbf{m}$ enough well. Therefore, we use reconstructed PCA models of an even lower dimension $l_2$ for training. 
% The supervised training of $f_W$ formulates as
% \begin{equation}
%     \argmin_{W}{||f_W(\hat{\mathbf{m}}_\text{pca}(\hat{\mathbf{\xi}}_{l_2}^i)) - \mathbf{m}^i||_1},
% \end{equation}


%xxx -- started editing again here

%% subsection 
\subsection{CNN-PCA Realizations and Flow Statistics}

Fig.~\ref{fig:petrel-reals} displays facies maps for three (reference) channelized realizations generated using Petrel. These models include six wells (two injectors and four producers), and conditioning data are available at all of these wells. The models contain $40 \times 40 \times 20$ grid blocks, with each block of dimensions $20$~m $\times$ 20~m $\times$ 2~m in the $x$, $y$ and $z$ directions.

%[xxx -- Add new Fig.~1 showing three Petrel realizations]

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-petrel-r1.pdf}
         \caption{}
         \label{real-3}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-petrel-r2.pdf}
         \caption{}
         \label{real-4}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-petrel-r3.pdf}
         \caption{}
         \label{real-5}
     \end{subfigure}
     
    
    \caption{Petrel realizations honoring facies data at the six wells. Black cylinders denote production wells, and white cylinders denote injection wells.}
    \label{fig:petrel-reals}
\end{figure}

The geomodels in Fig.~\ref{fig:petrel-reals} are characterized by 32,000 permeability values. As noted above, in the 3D CNN-PCA representation, the dimension of $\boldsymbol\xi$ ($l$) is set to 200. Fig.~\ref{fig:cnn-pca-reals} shows three realizations generated by the 3D CNN-PCA procedure. The resulting facies maps are thresholded such that the average facies proportions match those in the original Petrel models. The 3D CNN-PCA models display different channel connectivity patterns, with channel features (width, sinuosity) in approximate visual agreement with those in Fig.~\ref{fig:petrel-reals}.

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-cnnpca-case6.pdf}
         \caption{}
         \label{cnnpca-sat-p-eval}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-geo-true.pdf}
         \caption{}
         \label{cnnpca-true-model}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 4cm},clip, scale=0.3]{figs/chap2/3d-geo-r1.pdf}
         \caption{}
         \label{real-8}
     \end{subfigure}
    
    \caption{3D CNN-PCA realizations honoring facies data at the six wells.
    Model in (a) is used in the 3D recurrent R-U-Net assessment below. Model in (b) is the true model used in the history matching example. Black cylinders denote production wells, and white cylinders denote injection wells.}
    \label{fig:cnn-pca-reals}
\end{figure}

We now provide a quantitative assessment of the 3D CNN-PCA characterization by comparing flow results generated using these models to those from reference Petrel realizations. The well locations are shown in Figs.~\ref{fig:petrel-reals} and \ref{fig:cnn-pca-reals}, and the model dimensions are as noted above. One injector and two of the producers are completed in the top 10 layers, while the other injector and two producers are completed in the bottom 10 layers. The facies type for grid block~$i$ is denoted by $m_i$ ($m_i =1$ for sand and $m_i = 0$ for mud). The block permeability $k_i$ and porosity $\phi_i$ are related to facies type via $k_i = a\exp(b m_i)$ with $a = 20$~md and $b = \ln 100$, and $\phi_i = c\exp(d m_i)$ with $c=0.1$ and $d=\ln 2.5$. This gives $k_i = 2000$~md and $\phi_i = 0.25$ for grid blocks characterized as sand, and $k_i = 20$~md and $\phi_i = 0.1$ for those associated with mud. 

We simulate oil-water flow over a time frame of 1000~days, which is long enough to reach high field watercut. All wells operate under bottom-hole pressure (BHP) control, with injector BHPs set to 330~bar and producer BHPs to 310~bar. Oil-water relative permeability curves are shown in Fig.~\ref{fig:chap2-rel-perm}. At a pressure of 325~bar, oil viscosity is 1.14~cp. Water viscosity is 0.31~cp, independent of pressure. Oil and water densities are 787~kg/m$^3$ and 1038~kg/m$^3$, respectively, at reservoir conditions. The fluid properties and well settings are the same in all flow simulations presented in this paper.

%[xxx -- add figure showing rel perms]
\begin{figure}[htbp]
  \centering
  \includegraphics[scale=0.5]{figs/rel_perm.pdf}
  \caption{Oil-water relative permeability curves used in all simulations.}
  \label{fig:chap2-rel-perm}
\end{figure}


Fig.~\ref{fig:cnnpca-flow-statistics} presents $\text{P}_{10}$, $\text{P}_{50}$, and $\text{P}_{90}$ flow responses for field oil and water production rates. These results were all generated using Stanford's ADGPRS \cite{zhou2012parallel} flow simulator. Results are shown for 500 CNN-PCA realizations (black curves) and 500 reference Petrel realizations (red curves). The $\text{P}_{50}$ (solid) curves depict the median response at each time step, while the $\text{P}_{10}$ and $\text{P}_{90}$ (dashed) curves show the responses corresponding to the 10th and 90th percentiles. 

The results in Fig.~\ref{fig:cnnpca-flow-statistics} indicate that there is a reasonable degree of variability within the ensembles of geomodels. Specifically, we see that water production rate varies by over a factor of two between the $\text{P}_{10}$ and $\text{P}_{90}$ results at late time. Water breakthrough is also seen to occur over a wide range of times. Of most interest to us here, however, is the close agreement between flow results for the 3D CNN-PCA and Petrel geomodels. This is significant as it demonstrates that the 3D CNN-PCA procedure is able to generate an ensemble of models that provide detailed flow statistics that correspond to those associated with the reference set of geomodels. This suggests that, once it is trained based on reference Petrel realizations, 3D CNN-PCA can be used in place of Petrel to provide geomodels with the appropriate degree of variability.


\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/Field_OIL.png}
         \caption{Field Oil Rate}
         \label{pfs-orate-w1}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/Field_WAT.png}
         \caption{Field Water Rate}
         \label{pfs-wrate-w1}
     \end{subfigure}
    % \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{Field_WIR.png}
    %      \caption{Field Water Injection Rate}
    %      \label{pfs-wrate-w1}
    %  \end{subfigure}
    
    \caption{Flow statistics over ensembles of 500 new 3D CNN-PCA models and 500 new Petrel models. Solid curves correspond to $\text{P}_{50}$ results, lower and upper dashed curves to $\text{P}_{10}$ and $\text{P}_{90}$ results.}
    \label{fig:cnnpca-flow-statistics}
\end{figure}




\section{Recurrent R-U-Net Surrogate Model and Evaluations}

In this section, we first describe the 3D recurrent R-U-Net surrogate model along with the training setup. Results for global saturation and pressure fields are then shown. Finally, comparisons between surrogate model and high-fidelity simulation predictions for well flow rates, for both a single realization and an ensemble of new realizations, are presented.

\subsection{Recurrent R-U-Net Architecture and Training}

\textcolor{blue}{The 3D immiscible oil-water flow problem considered in this work is governed by mass conservation:
\begin{equation} 
    -\nabla \cdot (\rho_j v_j) - q_j^\text{w} = \frac{\partial}{\partial{t}}(\phi \rho_j S_j), \ \ \  j=o,~w.
\label{eq:mass-balance-eq}
\end{equation}
Here $j$ denotes phase, with $j = o$ representing oil phase and $w$ representing water phase, $\rho_j$ denotes phase density,  $q_j^\text{w}$ is the source/sink term (superscript $\text{w}$ indicates well), $t$ denotes time, $\phi$ denotes the rock porosity, $S_j$ is the phase saturation and $v_j$ is the phase velocity, which can be described by Darcy's law:
\begin{equation} 
     v_j =  -\frac{\mathbf{k} k_{rj}}{\mu_j} (\nabla p_j - \rho_j g \nabla z),
\label{eq:darcy-eq}
\end{equation}
where $\mathbf{k}$ is the absolute permeability tensor, $k_{rj}$ is the relative permeability, $\mu_j$ is phase viscosity, $p_j$ denotes the phase pressure, $g$ is the gravitational acceleration and $z$ denotes the depth. Here, $k_{rj}$ and $\mu_j$ are usually highly nonlinear functions of phase saturation $S_j$ and phase pressure $p_j$ respectively. }



In the context of history matching, many simulation runs must be performed \textcolor{blue}{to solve the discretized versions of Eq.~\ref{eq:mass-balance-eq} }with different geomodels~$\mathbf{m}$. We express a simulation run in this setting as
%
\begin{align}
    % \mathbf{x} = f(\mathbf{m}, \mathbf{u}),
    \mathbf{x} = f(\mathbf{m}),
    \label{eq-f}
\end{align}
%
where $f$ denotes the reservoir simulator and $\mathbf{x} \in \mathbb{R}^{n_b \times n_t}$ denotes the dynamic state fields. Here $n_b$ indicates the number of grid blocks and $n_t$ the number of time steps at which solution variables are predicted (here we take $n_t=10$, which is much less than the total number of time steps in the simulation). Because in this work we consider oil-water systems with capillary pressure neglected, $\mathbf{x}$ contains water saturation and pressure variables.




The 3D recurrent R-U-Net, illustrated in Fig.~\ref{fig:recurrent-r-u-net}, is applied to replace the expensive numerical simulation~$f$ in history matching scenarios. The recurrent R-U-Net consists of a 3D convolutional encoding net, a convolutional decoding net, and convLSTM neural networks~\citep{xingjian2015convolutional}. The encoding net extracts feature maps $\mathbf{F}_1$ to $\mathbf{F}_5$ from the input geomodel $\mathbf{m}$. Of these feature maps, $\mathbf{F}_5$ represents $\mathbf{m}$ in the most compressed manner. For this reason, $\mathbf{F}_5$ is propagated in time to provide feature representations of the state maps (i.e., we have $\mathbf{F}_5^1, \cdots, \mathbf{F}_5^{n_t}$) by the 3D convLSTM neural network. Combined with extracted local features $\mathbf{F}_1$ to $\mathbf{F}_4$, the propagated $\mathbf{F}_5^{t}$ $(t=1, \cdots, n_t)$ is upsampled to the corresponding (approximated) state map $\hat{\mathbf{x}}^{t}$ by the decoding net.

\textcolor{blue}{The 3D convLSTM net is the key module to capture the temporal dynamics of 3D high-dimensional systems. The convLSTM net effectively incorporates the advantage of LSTM~\citep{greff2016lstm} to capture the temporal evolution while maintaining the spatial information extracted by CNNs. The internal cell state $C^t$ in 3D convLSTM net carries the temporal-spatial information flow at time~$t$ and is updated by   
\begin{equation}
     \mathbf{C}^t = \mathbf{f}^t \circ \mathbf{C}^{t-1} + \mathbf{i}^t \circ \tilde{\mathbf{C}}^t,
 \end{equation}
 where forget gate $\mathbf{f}^t$ controls which information to discard from the previous cell state $\mathbf{C}^{t-1}$, input gate $\mathbf{i}^t$ decides which information to update from the new candidate cell state $\tilde{\mathbf{C}}^t$, and $\circ$ denotes the Hadamard product. The output state $\mathbf{H}^t$ at time~$t$ is computed based on $\mathbf{C}^t$ and is regulated by the output gate $\mathbf{o}^t$:
   \begin{equation}
     \mathbf{H}^t = \mathbf{o}^t \circ \tanh(\mathbf{C}^t),
 \end{equation}
where $\mathbf{o}^t$ filters which information in the cell state $\mathbf{C}^t$ is transferred to the output state $\mathbf{H}^t$.}

\textcolor{blue}{
The three operating gates $\mathbf{f}^t$, $\mathbf{i}^t$ and $\mathbf{o}^t$, as well as the new candidate cell state~$\tilde{\mathbf{C}}^t$ are determined from the previous output state $\mathbf{H}^{t-1}$ and the current input $\boldsymbol\chi^t$ following the expressions below:
 \begin{equation}
     \mathbf{f}^t = \sigma(\mathbf{W}_{xf} * {\boldsymbol\chi}^t + \mathbf{W}_{hf}*\mathbf{H}^{t-1} + \mathbf{b}_f),
 \end{equation}
  \begin{equation}
     \mathbf{i}^t = \sigma(\mathbf{W}_{xi} * {\boldsymbol\chi}^t + \mathbf{W}_{hi}*\mathbf{H}^{t-1} + \mathbf{b}_i),
 \end{equation}
  \begin{equation}
     \mathbf{o}^t = \sigma(\mathbf{W}_{xo} * {\boldsymbol\chi}^t + \mathbf{W}_{ho}*\mathbf{H}^{t-1} + \mathbf{b}_o),
 \end{equation}
  \begin{equation}
     \tilde{\mathbf{C}}^t = \tanh(\mathbf{W}_{xc} * {\boldsymbol\chi}^t + \mathbf{W}_{hc}*\mathbf{H}^{t-1} + \mathbf{b}_c),
 \end{equation}
where $\mathbf{W}$ and $\mathbf{b}$ are 3D convolution kernel weights and bias terms, which are shared across convLSTM cells. The parameters associated with these quantities are tuned during the training process.}

The detailed architectures of the encoding and decoding nets used in this work are the same as those described in \citep{tang2020deep}, with 2D convolutional kernels replaced with 3D convolutional kernels. \textcolor{blue}{And the detailed architecture illustration of the overall recurrent R-U-Net is provided in Appendix~A.2}. The combination of the convolutional and recurrent neural network architectures enables the surrogate model to accurately capture both spatial and temporal information in dynamic subsurface flow problems.

\begin{figure}[htbp]
  \centering
  \includegraphics[trim={2cm 2.5cm 1cm 2.5cm},clip, scale=0.6]{figs/convLSTM.pdf}
  \caption{Recurrent R-U-Net architecture incorporating 3D convLSTM into the R-U-Net~(\textcolor{blue}{detailed architecture illustration is provided in Appendix~A.2}. The combination of the convolutional and recurrent neural network architecture). Here the convLSTM net takes the global feature map $\mathbf{F}_5$ from the encoding net and generates a sequence of feature maps $\mathbf{F}_5^t$ $(t=1,\dots, n_t)$ that will be decoded into a sequence of state maps $\hat{\mathbf{x}}^{t}$ $(t=1,\dots, n_t)$ separately, using the same decoding net  (figure modified from \citep{tang2020deep}).}
  \label{fig:recurrent-r-u-net}
\end{figure}


The recurrent R-U-Net is trained using saturation and pressure solutions from 2500  simulation runs. The same simulation setup as was used for the 3D CNN-PCA flow assessment is applied here. The neural network parameters are tuned, in an automated manner, to minimize the $L^p$ norm of the difference between the recurrent R-U-Net output $\hat{\mathbf{x}}$ and the simulation reference $\mathbf{x}$. Specifically, training entails finding the tunable network parameters $\boldsymbol\theta$ via
%
\begin{equation}
\argmin_{\boldsymbol\theta} \frac{1}{n_s}\frac{1}{n_t} \sum_{i=1}^{n_s} \sum_{t=1}^{n_t} ||{\hat {\mathbf x}}^t_i - \mathbf{{x}}_{i}^{t}||_{p}^p + \lambda\frac{1}{n_s}\frac{1}{n_t}\frac{1}{n_\text{w}} \sum_{i=1}^{n_s} \sum_{t=1}^{n_t} \sum_{\text{w}=1}^{n_\text{w}} ||{\hat {x}}^{t, \text{w}}_{i} - {x}_{i}^{t, \text{w}}||_{p}^p.
\label{eq:loss-function}
\end{equation}
%
Here, $n_s$ denotes the number of training samples, $n_t$ indicates the number of time steps considered, and $n_w$ is the number of well blocks. The second term on the right-hand side of Eq.~\ref{eq:loss-function} acts to add weight (with weighting factor $\lambda$) to well-block quantities, indicated by superscript w. These values are important for predicting well rates, which are the primary quantities used in history matching. 

We found that better predictions of the global saturation and pressure fields were achieved by using the $L^2$ norm for saturation and the $L^1$ norm for pressure.  Therefore, two separate recurrent R-U-Nets are used in this work. We use a batch size of 8 and train each of the recurrent R-U-Nets for 260~epochs \textcolor{blue}{using Adam optimizer~\citep{kingma2014adam} with a learning rate decay schedule}. These trainings each require about 7~hours using a Tesla V100 GPU. As discussed in \cite{tang2020deep}, a single network, with appropriate (tuned) weights for the pressure and saturation losses, could also be used.

%%subsection
%\subsection{Data processing}

Proper data preparation and scaling contribute to the effective training of the recurrent R-U-Net. In this work, we use the same data pre-processing technique as described in \cite{tang2020deep}. Specifically, the input binary geomodel is naturally represented by facies block values (0 denotes mud and 1 denotes sand), and saturation maps are physically constrained between 0 and 1, so these sets of values are used directly. Pressure maps are normalized at each time step based on the maximum and minimum grid-block pressures observed at that time step in the high-fidelity simulation. We found this \textcolor{blue}{detrending} treatment to lead to better overall performance than normalization based on the time-invariant injector and producer BHPs. See \cite{tang2020deep} for details.


% The mean pressure map at time step $t$ is first computed by
%   \begin{equation}
%      \bar{\mathbf{p}}^{t} = \frac{1}{n_s}\sum_{i}^{n_s} \mathbf{p}^{t}_i \quad (t = 1, \dots, n_t).
%      \label{eq:p-0}
% \end{equation}

% Then the pressure data are centered around the origin for every time step~$t$ by 
%  \begin{equation}
%      \hat{\mathbf{p}}^{t}_i = \mathbf{p}^{t}_i - \bar{\mathbf{p}}^{t}, \quad i=1,\dots, n_s, \ \ t = 1, \dots, n_t.
%      \label{eq:p-1}
% \end{equation}

% Finally min-max normalization is performed on $\hat{\mathbf{p}}^{t}_i$ by applying 
% \begin{equation}   
%      \tilde{\mathbf{p}}^{t}_i = \frac{\hat{\mathbf{p}}^{t}_i - \text{min} ([\hat{\mathbf{p}}^{t}_1, \dots, \hat{\mathbf{p}}^{t}_{n_s}])}{\text{max} ([\hat{\mathbf{p}}^{t}_1, \dots, \hat{\mathbf{p}}^{t}_{n_s}]) - \text{min} ([\hat{\mathbf{p}}^{t}_1, \dots, \hat{\mathbf{p}}^{t}_{n_s}])},  \quad i=1,\dots, n_s, \ \ t = 1, \dots, n_t,
%      \label{eq:p-2}
%  \end{equation}
% where `max' and `min' find the maximum and minimum scalar values for all the training pressure maps at time step~$t$. This detrending process of pressure data was shown to improve the recurrent R-U-Net performance by our experiments.



% subsection
\subsection{Recurrent R-U-Net Evaluations}
\label{sect:saturation-pressure-map-eval}

A total of 400 new CNN-PCA geomodels (test cases) are used to evaluate the performance of the 3D recurrent R-U-Net. The surrogate model predicts pressure and saturation fields at $n_t=10$ time steps (50, 100, 150, 300, 400, 500, 600, 700, 850 and 1000~days). We first present predictions for saturation at three representative time steps, 50, 400 and 1000~days, for a single geomodel. This  geomodel, shown in Fig.~\ref{fig:cnn-pca-reals}(a), is characterized by saturation and pressure prediction errors (quantified below) that are near, but slightly greater than, the median errors over the 400 test cases. Thus we view this case as representative.

The predicted and reference saturation fields are shown in Fig.~\ref{fig:sat-map-single}.
%and \ref{fig:pressure-map-single}. 
The top row displays the recurrent R-U-Net 3D state map predictions and the bottom row shows the high-fidelity (ADGPRS) simulation results.
%and the bottom row shows the difference between those results.
The progress of the saturation front is, as expected, strongly impacted by the high-permeability channels. The 3D recurrent R-U-Net is able to capture the  evolution of the saturation field reasonably accurately, though some error is evident. Differences can be observed, for example, in the top layer, in the progress of the front originating from injector~I1 (compare Fig.~\ref{fig:sat-map-single}(c) to Fig.~\ref{fig:sat-map-single}(f)). We also see some water in the vicinity of producer~P2 in Fig.~\ref{fig:sat-map-single}(c) that does not appear in Fig.~\ref{fig:sat-map-single}(f). We note finally that the 3D aspect of the saturation field appears to be predicted accurately, as is evident from the cross-sectional views in Fig.~\ref{fig:sat-map-single}.

Because the global pressure field changes only slightly in time, instead of showing the evolution of pressure for a single realization, we instead present the pressure fields for three different test cases. These results are displayed in Fig.~\ref{fig:pressure-map-single}. All results are at 400~days. The global pressure fields for the three different realizations show significant differences, though the surrogate model provides an accurate visual 3D representation in all cases.

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-surr-1.pdf}
         \caption{50~days (surr)}
         \label{real-3}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-sur-2.pdf}
         \caption{400~days (surr)}
         \label{real-4}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-surr-3.pdf}
         \caption{1000~days (surr)}
         \label{real-5}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-sim-1.pdf}
         \caption{50~days (sim)}
         \label{real-6}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-sim-2.pdf}
         \caption{400~days (sim)}
         \label{real-7}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/3d-sat-sim-3.pdf}
         \caption{1000~days (sim)}
         \label{real-8}
     \end{subfigure}
    \caption{Saturation fields from 3D recurrent R-U-Net surrogate model (top row) and high-fidelity simulator (bottom row) at three different times.}
    %, along with difference maps (bottom row), at three different times.}
    \label{fig:sat-map-single}
\end{figure}



\begin{figure}[htbp]
     \centering
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-surr-day400-case6.pdf}
         \caption{Realization~1 (surr)}
         \label{real-3}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-surr-day400-r2.pdf}
         \caption{Realization~2 (surr)}
         \label{real-4}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-sim-day400-r1.pdf}
         \caption{Realization~3 (surr)}
         \label{real-5}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-sim-day400-case6.pdf}
         \caption{Realization~1 (sim)}
         \label{real-6}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-sim-day400-r2.pdf}
         \caption{Realization~2 (sim)}
         \label{real-7}
     \end{subfigure}
          \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={4.5cm 3.5cm 4cm 3cm},clip, scale=0.25]{figs/chap2/p-sim-day400-r1.pdf}
         \caption{Realization~3 (sim)}
         \label{real-8}
     \end{subfigure}
    \caption{Pressure maps from 3D recurrent R-U-Net surrogate model (top row) and high-fidelity simulator (bottom row) for three different test-case realizations. All results are at 400~days. Saturation results in Fig.~\ref{fig:sat-map-single} are for Realization~1, shown in Fig.~\ref{fig:cnn-pca-reals}(a).}
    \label{fig:pressure-map-single}
\end{figure}

In addition to visual comparisons, it is of interest to quantify the errors associated with the saturation and pressure predictions. We thus compute relative saturation and pressure errors, given as follows:
% 
\begin{equation}
%\delta_S = \frac{1}{n_{e}n_bn_{t}}\sum_{i=1}^{n_{e}}\sum_{j=1}^{n_b}\sum_{t=1}^{n_t} \frac{\norm{S_{i,j,t}^{surr} - S_{i,j,t}^{sim}}}{S_{i,j,t}^{sim}},
{\delta_S = \frac{1}{n_{e}n_b n_t}\sum_{i=1}^{n_{e}}\sum_{j=1}^{n_b}\sum_{t=1}^{n_t} \frac{\norm{{(\hat{S}_w)}_{i, j}^{t} - {(S_w)}_{i,j}^{t}}}{{(S_w)}_{i,j}^{t}}},
\label{eq:sat-relative-error-time-t}
\end{equation}
%

\begin{equation}
%\delta_p = \frac{1}{n_{e}n_bn_{t}}\sum_{i=1}^{n_{e}}\sum_{j=1}^{n_b}\sum_{t=1}^{n_t} \frac{\norm{p_{i,j,t}^{surr} - p_{i,j,t}^{sim}}}{p_{max}^{sim} - p_{min}^{sim}},
{\delta_p = \frac{1}{n_{e}n_b n_t}\sum_{i=1}^{n_{e}}\sum_{j=1}^{n_b}\sum_{t=1}^{n_t} \frac{\norm{\hat{p}_{i,j}^{t} - p_{i,j}^{t}}}{p_{i,\text{max}}^t - p_{i,\text{min}}^t}},
\label{eq:pressure-relative-error-time-t}
\end{equation}
%
where $n_e=400$ is the number of test models considered. All other variables are as defined previously. The denominator in Eq.~\ref{eq:sat-relative-error-time-t} is well behaved since the initial (and minimum) saturation is 0.1. %[xxx -- is 0.1 correct here?] Yes correct.

Applying Eqs.~\ref{eq:sat-relative-error-time-t} and \ref{eq:pressure-relative-error-time-t}, we obtain $\delta_S = 5.7\%$ and $\delta_p = 0.7\%$. These relatively low error values indicate that the 3D recurrent R-U-Net provides accurate global saturation and pressure predictions over the full ensemble of new geomodels. We next consider prediction accuracy in well-rate quantities.


\subsection{Predictions for Well Flow Rates}

Because well responses typically comprise the key data used in history matching, it is important to assess surrogate model accuracy for these quantities. In this work we consider 3D models with vertical wells that perforate multiple blocks. For well-block $i$, we compute well rates from the block states using the standard Peaceman model \citep{peaceman1983interpretation}:
%
\begin{equation}
\label{eq:well_flow}
    \left(q_j^\text{w}\right)_i = \text{WI}_i  (\lambda_j  \rho_j)_i (p - p^\text{w})_i.
\end{equation}
%
Here $j$ denotes the phase ($j = o$ for oil and $j = w$ for water), $\lambda_j=k_{rj}/\mu_j$ is the mobility of phase $j$ ($k_{rj}$ is the relative permeability to phase $j$ and $\mu_j$ is phase viscosity), $\rho_j$ is phase density, $p_i$ is well-block pressure, $p^\text{w}_i$ is the wellbore pressure in block $i$, and $\text{WI}_i$ is the well index in block $i$. The well index is computed from the well-block permeability and geometry, and the wellbore radius. 


For a vertical well with multiple perforations, the wellbore pressure $p^\text{w}_i$ varies in $z$ as a result of gravitational effects. Wellbore pressure at the first (uppermost) perforation is taken as the BHP. The wellbore pressure in the block below, $p^\text{w}_{i+1}$, is computed using %\cite{xxx} &&& should I cite the paper here?
%
\begin{equation}
\label{eq:standard-well}
    p^\text{w}_{i+1} = p^\text{w}_{i} + \rho_{i, i+1}g\Delta z_{i, i+1}.
\end{equation}
%
Here $\rho_{i, i+1}$ denotes the fluid mixture density between neighboring well-blocks $i$ and $i+1$, $g$ is gravitational acceleration, and $\Delta z_{i, i+1}$ is the depth difference. The fluid mixture density can be approximated based on the individual phase densities and the phase flow rates. See \citep{jiang2008techniques} for further details.

% The fluid mixture density is commonly approximated by the volume-weighted phase density at the nearest upstream perforation:
% \begin{equation}
%   \rho_{i, i+1} = \frac{\sum_{j = 1}^{n_p}(\rho_j q_j^{\text{w}} )_i }{\sum_{j = 1}^{n_p}( q_j^{\text{w}})_i},
% \end{equation}
% where $n_p$ denotes the total number of phases, and $(q_j^{\text{w}})_i$ is the volumetric rate at upstream perforation~$i$ that can be derived from Eq.~\ref{eq:well_flow}. Therefore, the well rates at different well grid blocks can be derived iteratively from the
% upstream to downstream perforations.

Well rates are computed, for both the surrogate model and the ADGPRS high-fidelity simulations, using the treatment described above. This procedure has been implemented in a standalone post-processing module. For the ADGPRS runs we could also use the well model in the simulator, which gives very similar results. To assure identical well-model treatments, however, we compute ADGPRS (HFS) well rates from the global simulation results using Eqs.~\ref{eq:well_flow} and \ref{eq:standard-well}.

Oil and water production rates for the four producers, as a function of time, are shown in Fig.~\ref{fig:producer-flow-single-case}. These results are for the 3D CNN-PCA geomodel shown in Fig.~\ref{fig:cnn-pca-reals}(a), with corresponding saturation fields shown in Fig.~\ref{fig:sat-map-single}. Results are generated at $n_t=10$ time steps, though in these and subsequent figures the points are connected linearly to provide continuous curves. The general level of agreement in well rates is quite close, and trends and water breakthroughs are captured with reasonable accuracy by the surrogate model. Slight discrepancies are apparent in some instances, however, such as in late-time water rate in Fig.~\ref{fig:producer-flow-single-case}(b) and (h).



We now present $\text{P}_{10}$, $\text{P}_{50}$ and $\text{P}_{90}$ oil and water production rates, evaluated over the 400 test cases. This assessment is analogous to that performed in our earlier evaluation of the geomodels provided by 3D CNN-PCA, though in that case all simulations were performed using ADGPRS. Results are shown in Fig.~\ref{fig:producer-flow-statistics}. The solid curves denote the $\text{P}_{50}$ well rates, while the lower and upper dashed curves indicate the $\text{P}_{10}$ and $\text{P}_{90}$ rates. Agreement in these statistical quantities is seen to be very close, which again demonstrates the accuracy of the surrogate model. It is noteworthy that accuracy is maintained over large ranges in rates, as is particularly evident in the water rate plots in Fig.~\ref{fig:producer-flow-statistics}.

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod1_orate.pdf}
         \caption{P1 oil rate}
         \label{pfs-case3-orate-w3}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod1_wrate.pdf}
         \caption{P1 water rate}
         \label{pfs-case3-wrate-w3}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod2_orate.pdf}
         \caption{P2 oil rate}
         \label{pfs-case3-orate-w5}
     \end{subfigure}
     %\hspace{1mm}
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod2_wrate.pdf}
         \caption{P2 water rate}
         \label{pfs-case3-wrate-w5}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod3_orate.pdf}
         \caption{P3 oil rate}
         \label{pfs-case3-orate-w11}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod3_wrate.pdf}
         \caption{P3 water rate}
         \label{pfs-case3-wrate-w11}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod4_orate.pdf}
         \caption{P4 oil rate}
         \label{pfs-case3-orate-w11}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod4_wrate.pdf}
         \caption{P4 water rate}
         \label{pfs-case3-wrate-w11}
     \end{subfigure}
    
    \caption{Comparison of oil (left) and water (right) production rates, for all four production wells, for the geomodel shown in Fig.~\ref{fig:cnn-pca-reals}(a). Red and black curves represent results from the 3D recurrent R-U-Net surrogate model and high-fidelity simulation, respectively.}
    \label{fig:producer-flow-single-case}
\end{figure}



\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod1_orate_ensemble.pdf}
         \caption{P1 oil rate}
         \label{pfs-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod1_wrate_ensemble.pdf}
         \caption{P1 water rate}
         \label{pfs-wrate-w1}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod2_orate_ensemble.pdf}
         \caption{P2 oil rate}
         \label{pfs-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod2_wrate_ensemble.pdf}
         \caption{P2 water rate}
         \label{pfs-wrate-w1}
     \end{subfigure}
     %\hfill
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod3_orate_ensemble.pdf}
         \caption{P3 oil rate}
         \label{pfs-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod3_wrate_ensemble.pdf}
         \caption{P3 water rate}
         \label{pfs-wrate-w1}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod4_orate_ensemble.pdf}
         \caption{P4 oil rate}
         \label{pfs-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap3/prod4_wrate_ensemble.pdf}
         \caption{P4 water rate}
         \label{pfs-wrate-w1}
     \end{subfigure}
     %\hfill
    
\caption{Comparison of oil (left) and water (right) production rate statistics, for all four production wells, over the full ensemble of 400 test cases. Red and black curves represent results from the recurrent R-U-Net surrogate model and high-fidelity simulation, respectively. Solid curves correspond to $\text{P}_{50}$ results, lower and upper dashed curves to $\text{P}_{10}$ and $\text{P}_{90}$ results.}
    \label{fig:producer-flow-statistics}
\end{figure}


\textcolor{blue}{The average relative errors in oil and water production rates across all production wells over all time steps, are quantified by
}
\begin{equation}
\textcolor{blue}{\delta_{r,j} = \frac{1}{n_{e}n_{p}n_t}\sum_{i=1}^{n_{e}}\sum_{k=1}^{n_p}\sum_{t=1}^{n_{t}} \frac{\norm{{(\hat{r}_{j})}_{i,k}^{t} - {({r}_{j})}_{i,k}^{t}}}{{({r}_{j})}_{i,k}^{t} + \epsilon}},
\label{eq:rate-rel-error-time-t}
\end{equation}
\textcolor{blue}{where $n_p$ denotes the number of production wells, ${(\hat{r}_{j})}_{i,k}^{t}$ denotes the phase ($j=o$ for oil and $w$ for water) production rate from the surrogate for well $k$ at time step~$t$ in test sample~$i$, and ${({r}_{j})}_{i,k}^{t}$ denotes the corresponding high-fidelity simulation results. A constant $\epsilon = 10$ is introduced in the denominator to avoid division by zero. Over $n_e = 400$ test samples, we have the relative errors for oil and water production rates: $\delta_{r,o} = 6.1\%$ and $\delta_{r,w} = 8.8\%$. The quantified relative errors are sufficiently small to enable the application of the introduced surrogate model in history matching.}


\section{Use of Deep-Learning Procedures for History Matching}

In this section, we apply 3D CNN-PCA and the 3D recurrent R-U-Net surrogate model for a challenging history matching problem \textcolor{blue}{ with two different history matching algorithms: a rigorous rejection sampling and an ensemble-based method.} In the application of 2D CNN-PCA in \cite{tang2020deep}, the low-dimensional variable $\boldsymbol\xi$ was optimized using a randomized maximum likelihood method to construct posterior geomodels. In \textcolor{blue}{rejection sampling},
%\textcolor{red}{this study}
the 3D CNN-PCA procedure is used only to provide a very large number of prior models; i.e., $\boldsymbol\xi$ is not manipulated to achieve a history match. We proceed in this manner because the rejection sampling algorithm used here does not involve any sort of optimization process. The generation of prior models using 3D CNN-PCA is much faster than it would typically be with geological modeling software. \textcolor{blue}{This low-dimensional variable $\boldsymbol\xi$ is updated, however, using ensemble smoother with multiple data assimilation, and 3D CNN-PCA effectively solves the curse of dimension issue in related algorithms. In the end, the ensemble-based history matching results are further evaluated by comparing with the rigorous rejection sampling posteriors. }

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well1.pdf}
         \caption{P1 oil rate}
         \label{hm-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well1.pdf}
         \caption{P1 water rate}
         \label{hm-wrate-w1}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well2.pdf}
         \caption{P2 oil rate}
         \label{hm-orate-w14}
     \end{subfigure}
     %\hspace{1mm}
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well2.pdf}
         \caption{P2 water rate}
         \label{hm-wrate-w14}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well3.pdf}
         \caption{P3 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well3.pdf}
         \caption{P3 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
     
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well4.pdf}
         \caption{P4 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well4.pdf}
         \caption{P4 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
    
    \caption{Oil (left) and water (right) production for all four production wells. Gray regions represent the prior $\text{P}_{10}$--$\text{P}_{90}$ range, red circles and curves denote observed and true data, and blue dashed curves denote the posterior $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) predictions. Vertical dashed line indicates the latest time at which data are collected.}
    \label{fig:hm-well-flow}
\end{figure}
\subsection{Rejection Sampling Algorithm}

Rejection sampling (RS) is a rigorous history matching algorithm that can be used to provide a reliable reference for posterior uncertainty. RS is usually very expensive computationally, however, as it requires generating and evaluating an extremely large number of prior samples. Thus the application of RS is clearly facilitated through the use of 3D CNN-PCA and the recurrent R-U-Net surrogate model. RS accepts or rejects prior samples independently, thus assuring that the accepted models are independent. In this work, we combine the RS approach described in \citep{sun2017new} with our deep-learning-based treatments. The overall workflow is as follows:
%
\begin{itemize}
    \item Sample the low-dimensional variable $\boldsymbol\xi \in \mathbb{R}^l$ from its prior distribution, given by $\mathcal{N}(\mathbf{\mu}_{\boldsymbol\xi}, C_{\boldsymbol\xi})$. Construct $\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)$ using CNN-PCA. 
    \item Sample a probability $p$ from a uniform distribution in $[0, 1]$.
    \item Compute the likelihood function $L(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi))$, given by 
    \begin{equation}
        L(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)) = c \text{exp}\left(-\frac{1}{2}[\hat{f}(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)) - \mathbf{d}_{\text{obs}}]^{\intercal}C_D^{-1}[\hat{f}(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)) - \mathbf{d}_{\text{obs}}]\right),
    \end{equation}
    where $c$ is a normalization constant, $\hat{f}(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi))$ indicates the surrogate model predictions for well rates for geomodel $\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)$,
    $\mathbf{d}_{\text{obs}}$ denotes the observed well rate data, and $C_D$ is the covariance matrix of data measurement error. 
    \item Accept $\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)$ if $p \leq \frac{L(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi))}{S_L}$, where $S_L$ is the maximum likelihood value over all prior models considered. 
\end{itemize}



\subsection{Problem Setup and \textcolor{blue}{Rejection Sampling Results} \textcolor{red}{History Matching Results}}


The `true' model considered here, which is shown in Fig.~\ref{fig:cnn-pca-reals}(b), is a randomly selected 3D CNN-PCA realization. Recall that all realizations (including the true model) are conditioned to hard data at well locations. The true data $\mathbf{d}_{\text{true}}$ are obtained by performing high-fidelity simulation using the true geomodel. The observed data $\mathbf{d}_{\text{obs}}$ comprise the true data with random error added
%
\begin{equation}
\mathbf{d}_{\text{obs}} = \mathbf{d}_{\text{true}} + \boldsymbol\epsilon,
\end{equation}
%
where $\boldsymbol\epsilon$ is the measurement error vector, with all components taken to be Gaussian random variables with mean of zero and covariance consistent with the $C_D$ matrix defined above. 

\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 3cm},clip, scale=0.3]{figs/chap4/rs-pos-1.pdf}
         \caption{}
         \label{real-3}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 3cm},clip, scale=0.3]{figs/chap4/rs-pos-2.pdf}
         \caption{}
         \label{real-4}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim={7cm 5cm 5cm 3cm},clip, scale=0.3]{figs/chap4/rs-pos-3.pdf}
         \caption{}
         \label{real-5}
     \end{subfigure}

    \caption{Three (randomly selected) 3D CNN-PCA realizations accepted by the rejection sampling procedure.}
    \label{fig:rs-posterior}
\end{figure}




\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well_hfs_comp1.pdf}
         \caption{P1 oil rate}
         \label{hm-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well_hfs_comp1.pdf}
         \caption{P1 water rate}
         \label{hm-wrate-w1}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well_hfs_comp2.pdf}
         \caption{P2 oil rate}
         \label{hm-orate-w14}
     \end{subfigure}
     %\hspace{1mm}
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well_hfs_comp2.pdf}
         \caption{P2 water rate}
         \label{hm-wrate-w14}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well_hfs_comp3.pdf}
         \caption{P3 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well_hfs_comp3.pdf}
         \caption{P3 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
     
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_oil_well_hfs_comp4.pdf}
         \caption{P4 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/rs_151_accepted_hm_water_well_hfs_comp4.pdf}
         \caption{P4 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
    
    \caption{Oil (left) and water (right) production for all four production wells. Gray regions represent the prior $\text{P}_{10}$--$\text{P}_{90}$ range, blue dashed curves denote surrogate model posterior $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) predictions, red dashed curves denote high-fidelity simulation posterior $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) predictions. Vertical dashed line indicates the latest time at which data are collected.}
    \label{fig:hm-well-flow-comp}
\end{figure}


With RS, very few models will be accepted if we attempt to match a large number of data points, particularly if data error is small. Therefore, we use data at only two time steps, specifically at day~100 and day~150. Oil and water production rates are collected at the four producers, which means we have a total of 16 observations. The standard deviation of the measurement error is set to 15\% of the corresponding true data. One million prior models are generated using CNN-PCA. The 3D recurrent R-U-Net is then applied to provide well response predictions for all of these models. The generation of $10^6$ 3D CNN-PCA models requires about 3~hours, and the $10^6$ surrogate model predictions require about 8~hours. We estimate that high-fidelity simulation for these $10^6$ models would require about 170,000~hours of serial computation (as each HFS requires around 10~minutes). A total of 151 (out of $10^6$) models are accepted by the RS procedure.




The history matching results using this procedure are shown in Fig.~\ref{fig:hm-well-flow}. The gray areas display the $\text{P}_{10}$-$\text{P}_{90}$ interval for the prior models. The red points and curves denote the observed data and the true model flow response. The blue dashed curves indicate the $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) posterior RS results.

The posterior $\text{P}_{10}$--$\text{P}_{90}$ ranges are in most cases significantly smaller than the prior $\text{P}_{10}$--$\text{P}_{90}$ ranges. For this reason, predictions based on the posterior models would be expected to be much more useful than prior forecasts. It is evident that the posterior uncertainty ranges cover the true well responses even when these results are on the edge of the prior $\text{P}_{10}$-$\text{P}_{90}$ interval, e.g., the P2 oil rate at late time (Fig.~\ref{fig:hm-well-flow}(c)). We also see that the posterior predictions result in significant uncertainty reduction in P1 and P2 water rates (Fig.~\ref{fig:hm-well-flow}(b) and (d)), even though water production at these wells has not yet occurred at day~150.



In Fig.~\ref{fig:rs-posterior} we present three of the realizations accepted by the RS procedure. These realizations all show a lack of connectivity (through sand) between injector I1 and producer P2, at least in the layers that are visible in these images. This is consistent with the true 3D CNN-PCA model (shown in Fig.~\ref{fig:cnn-pca-reals}(b)) and with the low water production rates in Fig.~\ref{fig:hm-well-flow}(d). We also see that injector I2 is connected to producer P3 through sand in all three posterior realizations. This is again consistent with the true model, and with the early breakthrough and high water production rates in P3, evident in Fig.~\ref{fig:hm-well-flow}(f).


Finally, we simulate the 151 models accepted by RS using the high-fidelity simulator ADGPRS. 
%This allows us to further assess the applicability of our history matching procedure for this problem. 
Results for oil and water production for the four producers are shown in Fig.~\ref{fig:hm-well-flow-comp}. There we see very close agreement between the recurrent R-U-Net posterior predictions (blue dashed curves) and the high-fidelity simulation posterior predictions (red dashed curves). This is an important validation, as it demonstrates that the posterior models found using the 3D recurrent R-U-Net flow surrogate indeed correspond to HFS models that match the observed data. This clearly establishes the applicability of the 3D recurrent R-U-Net for this challenging history matching problem.

\textcolor{blue}{\subsection{Ensemble Smoother with Multiple Data Assimilation and Results }}

\textcolor{blue}{Ensemble smoother with multiple data assimilation~(ES-MDA)~\citep{emerick2013ensemble} is an iterative form of ensemble smoother~(ES)~\citep{evensen2000ensemble} and breaks the single global update of ES into multiple data assimilation steps. To guarantee the same posterior mean and covariance can be achieved between single and multiple data assimilation in linear-Gaussian cases, ES-MDA perturbs observations according to the inflated data covariance matrix at each data assimilation step. ES-MDA has demonstrated to be an efficient alternative for history matching algorithms with high computational cost, though its validity needs cautious evaluation as its posterior quantification is not mathematically supported for complex nonlinear problems and it can experience near ensemble collapse~\citep{morzfeld2017collapse}.}


\textcolor{blue}{
To demonstrate the capability of the introduced deep learning-based parameterization and surrogate modeling techniques on updating/optimizing parameterized variables, we combine 3D CNN-CPA and recurrent R-U-Net with ES-MDA. However, it is worth noting that it is not computationally efficient to do so in practice. Because the training samples required for the recurrent R-U-Net is in the equivalent magnitude of the total number of simulations needed in ES-MDA. Still, by combining 3D CNN-PCA and recurrent R-U-Net with ES-MDA, we are also able to provide consistent comparison of history matching results between ES-MDA and rejection sampling. The overall workflow of deep learning-assisted ES-MDA can be described as follows:}
\begin{enumerate}
    \item \textcolor{blue}{Select the number of data assimilations~$N_a$ and corresponding inflation coefficients~$\alpha_i$~$(i = 1, \cdots, N_a)$ where $\sum_{i = 1}^{N_a} \alpha_i = 1$, and select $N_e$ ensemble members.}
\end{enumerate}

\textcolor{blue}{
For each ensemble member:}

\begin{enumerate}[resume]

    \item \textcolor{blue}{Sample the low-dimensional variable $\boldsymbol\xi \in \mathbb{R}^l$ from its prior distribution~$\mathcal{N}(\mathbf{\mu}_{\boldsymbol\xi}, C_{\boldsymbol\xi})$.}
    \item \textcolor{blue}{For $i=1,\cdots, N_a$:}
    \textcolor{blue}{
    \begin{itemize}
    \item Construct $\mathbf{m}_{\text{cnn}}(\boldsymbol\xi)$ using CNN-PCA and obtain surrogate predictions $\hat{f}(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi))$. 
    \item Perturb the observation data by $\mathbf{d}_{\text{uc}} = \mathbf{d}_{\text{obs}} + \sqrt{\alpha_i}C_D^{1/2}z_d $ and $z_d \sim \mathcal{N}(0, I)$.
    \item Update lower-dimension variable $\boldsymbol\xi$ by
    \begin{equation}
       \boldsymbol\xi = \boldsymbol\xi + C_{MD}(C_{DD} + \alpha_i C_D)^{-1}( \mathbf{d}_{\text{uc}} - \hat{f}(\mathbf{m}_{\text{cnn}}( \boldsymbol\xi))),
    \end{equation}
    where $C_{MD}$ is the cross-covariance matrix between the before-update variable $\boldsymbol\xi$ and predicted data $\hat{f}(\mathbf{m}_{\text{cnn}}(\boldsymbol\xi))$, $C_{DD}$ is the auto-covariance matrix of the predicted data, and $C_D$ is the covariance matrix of data measurement error. 
    \end{itemize}}
\end{enumerate}



\begin{figure}[htbp]
     \centering
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_oil_well_paper1.pdf}
         \caption{P1 oil rate}
         \label{hm-orate-w1}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_water_well_paper1.pdf}
         \caption{P1 water rate}
         \label{hm-wrate-w1}
     \end{subfigure}
     %\hfill
     
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_oil_well_paper2.pdf}
         \caption{P2 oil rate}
         \label{hm-orate-w14}
     \end{subfigure}
     %\hspace{1mm}
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_water_well_paper2.pdf}
         \caption{P2 water rate}
         \label{hm-wrate-w14}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_oil_well_paper3.pdf}
         \caption{P3 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_water_well_paper3.pdf}
         \caption{P3 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
     
     
    \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_oil_well_paper4.pdf}
         \caption{P4 oil rate}
         \label{hm-orate-w17}
     \end{subfigure}
          \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/chap4/hm_methods_comp_water_well_paper4.pdf}
         \caption{P4 water rate}
         \label{hm-wrate-w17}
     \end{subfigure}
    
    \caption{Oil (left) and water (right) production for all four production wells. Gray regions represent the prior $\text{P}_{10}$--$\text{P}_{90}$ range, blue dashed curves denote rejection sampling posterior $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) predictions, red dashed curves denote ES-MDA posterior $\text{P}_{10}$ (lower), $\text{P}_{50}$ (middle) and $\text{P}_{90}$ (upper) predictions. Vertical dashed line indicates the latest time at which data are collected.}
    \label{fig:hm-well-flow-comp-edmda}
\end{figure}
\textcolor{blue}{
We select 200 ensemble members and specifies 10 steps of data assimilation. Meanwhile, the same observed data~(16 observations) and standard deviation of the measurement error as those used in rejection sampling are adopted. And the deep learning-assisted ES-MDA quantifies the posterior well response distributions by these 200 updated ensemble members. }
\textcolor{blue}{The comparison of history matching results between ES-MDA and rejection sampling is presented in Fig.~\ref{fig:hm-well-flow-comp-edmda}. We can observe that ES-MDA is able to provide posterior estimations of many well quantities that are in agreement with rejection sampling in the 3D channelized system setup, though it tends to overshoot the uncertainty for some well quantities, as illustrated by Figs.~\ref{fig:hm-well-flow-comp-edmda}(c), (d) and (f). The agreement, however, only suggests that ES-MDA with careful selection of inflation coefficients delivers acceptable posterior quantification for the 
presented flow model. Careful evaluations of ES-MDA posteriors are still required for other history matching problems with different flow models, and 3D CNN-PCA and recurrent R-U-Net provides an efficient means to achieve that purpose. }



%section
\section{Concluding Remarks}

In this work, CNN-PCA, a deep-learning-based geological parameterization technique, and the recurrent R-U-Net surrogate model for flow prediction, were extended to treat 3D systems. The 3D CNN-PCA method uses a supervised learning training strategy and was shown to provide 3D channelized models in general visual agreement with reference geomodels. Importantly, flow statistics based on ensembles of CNN-PCA models and reference Petrel models were demonstrated to be in close agreement, suggesting that the CNN-PCA realizations possess channel features and connectivity consistent with that in the reference models.

The 3D recurrent R-U-Net was shown to capture the saturation and pressure evolution accurately for 3D channelized models generated using CNN-PCA. This was established both visually and through aggregate error statistics. Time-varying well responses for vertical wells perforated in multiple blocks were also assessed. Recurrent R-U-Net well responses for a particular realization, in addition to well-flow-rate statistics evaluated over the full set of 400 test cases, were shown to agree closely with reference high-fidelity simulation results.

The deep-learning-based treatments were then used, in combination, for history matching. Rejection sampling was \textcolor{blue}{first} applied, with new (proposed) models generated very efficiently using 3D CNN-PCA, and evaluated in terms of flow response using the 3D recurrent R-U-Net. A total of $10^6$ models were generated and evaluated (which would have been extremely time consuming using geological modeling software and HFS), and 151 were accepted, for the problem considered. Significant uncertainty reduction was achieved, and high-fidelity simulation of the accepted geomodels provided results that closely tracked predictions from the 3D recurrent R-U-Net. \textcolor{blue}{ES-MDA was then applied with updated model variables parameterized by 3D CNN-PCA and flow quantities predicted by 3D recurrent R-U-Net for the purpose of consistent comparison with rejection sampling results. This further demonstrates the capability of the introduced parameterization and surrogate model to combine with optimization-based history matching algorithms.  }  

There are many important directions that should be considered in future work in this general area. A key challenge is the extension of the methods presented here to practical models containing, e.g., $O(10^6-10^7)$ cells. Because training time can scale with problem size, this may require the development and evaluation of different network architectures. It will also be of interest to extend our surrogate flow model to treat coupled flow-geomechanics systems. These problems can be very expensive to simulate, so surrogate models could be highly useful in this context. Finally, a wide range of history matching algorithms, including those considered too expensive for use in traditional settings, can be evaluated and compared using our deep-learning-based parameterization and surrogate flow modeling capabilities.


\section{Acknowledgements}
We are grateful to the Stanford Smart Fields Consortium and to Stanford--Chevron CoRE for partial funding of this work. We also thank the Stanford Center for Computational Earth \& Environmental Science (CEES) for providing computational resources.

% \begin{thebibliography}{6pt}
%   \bibitem[{<reference>}]{<cite>} ...
% \end{thebibliography}
%

